Cityscape-Adverse: Benchmarking Robustness of Semantic Segmentation with Realistic Scene Modifications via Diffusion-Based Image Editing

Recent advancements in generative AI, particularly diffusion-based image editing, have enabled the transformation of images into highly realistic scenes using only text instructions. This technology offers significant potential for generating diverse synthetic datasets to evaluate model robustness. In this paper, we introduce Cityscape-Adverse, a benchmark that employs diffusion-based image editing to simulate eight adverse conditions, including variations in weather, lighting, and seasons, while preserving the original semantic labels. We evaluate the reliability of diffusion-based models in generating realistic scene modifications and assess the performance of state-of-the-art CNN and Transformer-based semantic segmentation models under these challenging conditions. Additionally, we analyze which modifications have the greatest impact on model performance and explore how training on synthetic datasets can improve robustness in real-world adverse scenarios. Our results demonstrate that all tested models, particularly CNN-based architectures, experienced significant performance degradation under extreme conditions, while Transformer-based models exhibited greater resilience. We verify that models trained on Cityscape-Adverse show significantly enhanced resilience when applied to unseen domains. Code and datasets will be released at https://github.com/naufalso/cityscape-adverse.

==> tables/acdc_evaluation_old.tex <==
% \begin{table*}[]
% \centering
% \caption{Performance Comparison of CNN and Transformer-based Models Trained on Different Configurations (CS, CSAdv, and CS,CSAdv) Evaluated on ACDC Adverse Conditions. The table presents the mIoU scores for each model across clean, snow, rain, fog, and night conditions, along with the average mIoU across all adverse conditions (adv.avg).}
% \label{tab:acdc-results}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|c|cccc|c|l|l|c|cccc|c|}
% \hline
% \multirow{2}{*}{\shortstack{Model Name\\(CNN)}} & \multirow{2}{*}{Trained On} & \multicolumn{6}{c|}{ACDC (Val) - mIoU} & \multirow{2}{*}{\shortstack{Model Name\\(Transformers)}} & \multirow{2}{*}{Trained On} & \multicolumn{6}{c|}{ACDC (Val) - mIoU} \\ \cline{3-8} \cline{11-16}
%                             &                             & clean          & snow           & rain           & fog            & night          & adv.avg          &                                     &             & clean          & snow           & rain           & fog            & night          & adv.avg \\ \hline
% \multirow{3}{*}{DeepLabV3+} & CS                          & 58.8           & 44.3           & 50.3           & 63.7           & 12.2           & 42.6             & \multirow{3}{*}{SegFormer}          & CS          & 57.2           & 51.2           & \textbf{52.7}  & 67.1           & 18.5           & 47.4    \\ 
%                             & CSAdv                       & 62.4           & 49.3           & \textbf{50.7}  & \textbf{64.9}  & \textbf{30.7}  & \textbf{48.9}    &                                     & CSAdv       & \textbf{60.9}  & \textbf{54.7}  & 49.6           & \textbf{69.3}  & \textbf{34.6}  & \textbf{52.1}    \\ 
%                             & CS,CSAdv                    & \textbf{63.5}  & \textbf{50.8}  & 49.7           & 62.7           & 30.3           & 48.4             &                                     & CS,CSAdv    & 60.7           & 53.5           & 49.8           & \textbf{69.3}  & 32.1           & 51.2    \\ \hline
                            
% \multirow{3}{*}{ICNet}      & CS                          & \textbf{61.2}  & 45.4           & 49.2           & 64.8           & 24.6           & 46.0             & \multirow{3}{*}{Mask2Former}        & CS          & 67.5           & 55.4           & 58.2           & \textbf{73.8}  & 31.4           & 54.7    \\
%                             & CSAdv                       & \textbf{61.2}  & \textbf{53.4}  & 50.3           & 65.1           & \textbf{38.3}  & \textbf{51.8}    &                                     & CSAdv       & \textbf{69.8}  & 61.6           & \textbf{58.6}  & 72.9           & 42.8           & \textbf{59.0}    \\
%                             & CS,CSAdv                    & 59.8           & 53.4           & \textbf{50.6}  & \textbf{66.1}  & 35.9           & 51.5             &                                     & CS,CSAdv    & 68.7           & \textbf{62.4}  & 55.3           & 73.0           & \textbf{43.7}  & 58.6    \\ \hline
                            
% \multirow{3}{*}{DDRNet}     & CS                          & 58.4           & 42.5           & 48.0           & 64.5           & 10.6           & 41.4             & \multirow{3}{*}{SETR}               & CS          & 60.7           & 55.6           & 58.3           & 70.1           & 38.1           & 55.5    \\
%                             & CSAdv                       & 59.1           & 44.3           & 49.0           & \textbf{65.8}  & \textbf{34.8}  & 48.5             &                                     & CSAdv       & \textbf{65.5}  & 61.7           & 58.0           & \textbf{74.9}  & \textbf{43.9}  & \textbf{59.6}    \\ 
%                             & CS,CSAdv                    & \textbf{61.2}  & \textbf{47.5}  & \textbf{51.3}  & 65.1           & 34.1           & \textbf{49.5}    &                                     & CS,CSAdv    & 64.6           & \textbf{62.2}  & \textbf{59.6}  & 73.9           & 40.9           & 59.1    \\ \hline
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Performance Comparison of CNN and Transformer-based Models Trained on Different Configurations (CS, CSAdv, and CS,CSAdv) Evaluated on ACDC Adverse Conditions. The table presents the mIoU scores for each model across clean, snow, rain, fog, and night conditions, along with the average mIoU across all adverse conditions (adv.avg).}
% \label{tab:acdc-results}
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|c|cccc|c|}
% \hline
% \textbf{Model Name} & \textbf{Trained On} & \textbf{Clean} & \textbf{Snow} & \textbf{Rain} & \textbf{Fog} & \textbf{Night} & \textbf{Adv. Avg} \\ \hline
% \multirow{3}{*}{DeepLabV3+} 
%     & CS          & 58.8  & 44.3  & 50.3  & 63.7  & 12.2  & 42.6 \\  
%     & CSAdv       & 62.4  & 49.3  & \textbf{50.7}  & \textbf{64.9}  & \textbf{30.7}  & \textbf{48.9} \\  
%     & CS,CSAdv    & \textbf{63.5}  & \textbf{50.8}  & 49.7  & 62.7  & 30.3  & 48.4 \\ \hline

% \multirow{3}{*}{ICNet} 
%     & CS          & \textbf{61.2}  & 45.4  & 49.2  & 64.8  & 24.6  & 46.0 \\  
%     & CSAdv       & \textbf{61.2}  & \textbf{53.4}  & 50.3  & 65.1  & \textbf{38.3}  & \textbf{51.8} \\  
%     & CS,CSAdv    & 59.8  & 53.4  & \textbf{50.6}  & \textbf{66.1}  & 35.9  & 51.5 \\ \hline

% \multirow{3}{*}{DDRNet} 
%     & CS          & 58.4  & 42.5  & 48.0  & 64.5  & 10.6  & 41.4 \\  
%     & CSAdv       & 59.1  & 44.3  & 49.0  & \textbf{65.8}  & \textbf{34.8}  & 48.5 \\  
%     & CS,CSAdv    & \textbf{61.2}  & \textbf{47.5}  & \textbf{51.3}  & 65.1  & 34.1  & \textbf{49.5} \\ \hline

% \multirow{3}{*}{SegFormer} 
%     & CS          & 57.2  & 51.2  & \textbf{52.7}  & 67.1  & 18.5  & 47.4 \\  
%     & CSAdv       & \textbf{60.9}  & \textbf{54.7}  & 49.6  & \textbf{69.3}  & \textbf{34.6}  & \textbf{52.1} \\  
%     & CS,CSAdv    & 60.7  & 53.5  & 49.8  & \textbf{69.3}  & 32.1  & 51.2 \\ \hline

% \multirow{3}{*}{Mask2Former} 
%     & CS          & 67.5  & 55.4  & 58.2  & \textbf{73.8}  & 31.4  & 54.7 \\  
%     & CSAdv       & \textbf{69.8}  & 61.6  & \textbf{58.6}  & 72.9  & 42.8  & \textbf{59.0} \\  
%     & CS,CSAdv    & 68.7  & \textbf{62.4}  & 55.3  & 73.0  & \textbf{43.7}  & 58.6 \\ \hline

% \multirow{3}{*}{SETR} 
%     & CS          & 60.7  & 55.6  & 58.3  & 70.1  & 38.1  & 55.5 \\  
%     & CSAdv       & \textbf{65.5}  & 61.7  & 58.0  & \textbf{74.9}  & \textbf{43.9}  & \textbf{59.6} \\  
%     & CS,CSAdv    & 64.6  & \textbf{62.2}  & \textbf{59.6}  & 73.9  & 40.9  & 59.1 \\ \hline
% \end{tabular}
% % }
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Performance Comparison of CNN and Transformer-based Models Trained on Different Configurations (CS: Cityscapes \cite{cordts2016cityscapes}, CSCnet: Cityscape-ControlNet \cite{loiseau2023reliability}, CS+CSCNet: Cityscape with Cityscape-ControlNet \cite{loiseau2023reliability}, CSAdv: Cityscapes-Adverse (Ours), and CS+CSAdv: Cityscape with Cityscape-Adverse (Ours). Evaluated on ACDC Adverse Conditions. The table presents the mIoU scores for each model across clean, snow, rain, fog, and night conditions, along with the average mIoU across all adverse conditions (adv.avg).}


% ===== New table without performance enhancements =====
% \label{tab:acdc-results}
% \begin{tabular}{|l|l|c|cccc|c|}
% \toprule
% \textbf{Model Name} & \textbf{Trained On} & \textbf{Clean} & \textbf{Snow} & \textbf{Rain} & \textbf{Fog} & \textbf{Night} & \textbf{Adv. Avg} \\ \midrule
% \multirow{5}{*}{DeepLabV3+} 
%     & CS \cite{cordts2016cityscapes}              & 58.8  & 44.3  & 50.3  & 63.7  & 12.2  & 42.6 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 39.9  & 26.8  & 33.7  & 45.8  & 15.0  & 30.3 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 47.4  & 35.8  & 41.7  & 51.9  & 20.1  & 37.4 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & 62.4  & 49.3  & \textbf{50.7}  & \textbf{64.9}  & \textbf{30.7}  & \textbf{48.9} \\  
%     & CS+CSAdv (Ours)        & \textbf{63.5}  & \textbf{50.8}  & 49.7  & 62.7  & 30.3  & 48.4 \\ \midrule

% \multirow{5}{*}{ICNet} 
%     & CS \cite{cordts2016cityscapes}              & \textbf{61.2}  & 45.4  & 49.2  & 64.8  & 24.6  & 46.0 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 38.8  & 28.3  & 33.4  & 48.0  & 16.7  & 31.6 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 49.7  & 34.8  & 41.8  & 51.3  & 22.5  & 37.6 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & \textbf{61.2}  & 53.4  & 50.3  & 65.1  & \textbf{38.3}  & \textbf{51.8} \\  
%     & CS+CSAdv (Ours)        & 59.8  & \textbf{53.4}  & \textbf{50.6}  & \textbf{66.1}  & 35.9  & 51.5 \\ \midrule

% \multirow{5}{*}{DDRNet} 
%     & CS \cite{cordts2016cityscapes}              & 58.4  & 42.5  & 48.0  & 64.5  & 10.6  & 41.4 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 34.1  & 24.0  & 30.3  & 41.5  & 16.8  & 28.2 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.4  & 36.2  & 40.5  & 52.2  & 21.7  & 37.7 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & 59.1  & 44.3  & 49.0  & \textbf{65.8}  & \textbf{34.8}  & 48.5 \\  
%     & CS+CSAdv (Ours)        & \textbf{61.2}  & \textbf{47.5}  & \textbf{51.3}  & 65.1  & 34.1  & \textbf{49.5} \\ \midrule

% \multirow{5}{*}{SegFormer} 
%     & CS \cite{cordts2016cityscapes}              & 57.2  & 51.2  & \textbf{52.7}  & 67.1  & 18.5  & 47.4 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 38.6  & 29.6  & 35.1  & 47.7  & 17.4  & 32.5 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 46.9  & 35.6  & 42.0  & 51.0  & 22.1  & 37.7 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & \textbf{60.9}  & \textbf{54.7}  & 49.6  & \textbf{69.3}  & \textbf{34.6}  & \textbf{52.1} \\  
%     & CS+CSAdv (Ours)        & 60.7  & 53.5  & 49.8  & \textbf{69.3}  & 32.1  & 51.2 \\ \midrule

% \multirow{5}{*}{Mask2Former} 
%     & CS \cite{cordts2016cityscapes}              & \textbf{67.5}  & 55.4  & 58.2  & \textbf{73.8}  & 31.4  & 54.7 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 39.3  & 32.8  & 38.4  & 52.0  & 24.9  & 37.0 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.4  & 39.3  & 45.1  & 53.9  & 28.3  & 41.7 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & \textbf{69.8}  & 61.6  & \textbf{58.6}  & 72.9  & 42.8  & \textbf{59.0} \\  
%     & CS+CSAdv (Ours)        & 68.7  & \textbf{62.4}  & 55.3  & 73.0  & \textbf{43.7}  & 58.6 \\ \midrule

% \multirow{5}{*}{SETR} 
%     & CS \cite{cordts2016cityscapes}              & 60.7  & 55.6  & 58.3  & 70.1  & 38.1  & 55.5 \\ \cmidrule{2-8}
%     & CSCnet \cite{loiseau2023reliability}          & 40.9  & 34.1  & 37.8  & 48.7  & 26.2  & 36.7 \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 49.1  & 40.6  & 46.2  & 52.7  & 30.5  & 42.5 \\ \cmidrule{2-8}
%     & CSAdv (Ours)           & \textbf{65.5}  & 61.7  & 58.0  & \textbf{74.9}  & \textbf{43.9}  & \textbf{59.6} \\  
%     & CS+CSAdv (Ours)        & 64.6  & \textbf{62.2}  & \textbf{59.6}  & 73.9  & 40.9  & 59.2 \\ \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Performance Comparison of CNN and Transformer-based Models Trained on Different Configurations (CS: Cityscapes \cite{cordts2016cityscapes}, CSCnet: Cityscape-ControlNet \cite{loiseau2023reliability}, CS+CSCNet: Cityscape with Cityscape-ControlNet \cite{loiseau2023reliability}, CSAdv: Cityscapes-Adverse (Ours), and CS+CSAdv: Cityscape with Cityscape-Adverse (Ours). Evaluated on ACDC Adverse Conditions. The table presents the mIoU scores for each model across clean, snow, rain, fog, and night conditions, along with the average mIoU across all adverse conditions (Adv. Avg). The values in pare\label{tab:acdc-results}
% \begin{tabular}{|l|l|cc|cc|cc|cc|cc|cc|}
% \toprule
% \textbf{Model Name} & \textbf{Trained On} & \multicolumn{2}{c|}{\textbf{Clean}} & \multicolumn{2}{c|}{\textbf{Snow}} & \multicolumn{2}{c|}{\textbf{Rain}} & \multicolumn{2}{c|}{\textbf{Fog}} & \multicolumn{2}{c|}{\textbf{Night}} & \multicolumn{2}{c|}{\textbf{Adv. Avg}} \\ \midrule
%  &  & \textbf{mIoU} & \textbf{Enh.} & \textbf{mIoU} & \textbf{Enh.} & \textbf{mIoU} & \textbf{Enh.} & \textbf{mIoU} & \textbf{Enh.} & \textbf{mIoU} & \textbf{Enh.} & \textbf{mIoU} & \textbf{Enh.} \\ \midrule

% \multirow{5}{*}{DeepLabV3+} 
%     & CS \cite{cordts2016cityscapes}              & 58.8  & (0.0)  & 44.3  & (0.0)  & 50.3  & (0.0)  & 63.7  & (0.0)  & 12.2  & (0.0)  & 42.6  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 39.9  & (-18.9)  & 26.8  & (-17.5)  & 33.7  & (-16.6)  & 45.8  & (-17.9)  & 15.0  & (2.8)  & 30.3  & (-12.3) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 47.4  & (-11.4)  & 35.8  & (-8.5)  & 41.7  & (-8.6)  & 51.9  & (-11.8)  & 20.1  & (7.9)  & 37.4  & (-5.3) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & 62.4  & (3.6)  & 49.3  & (5.0)  & \textbf{50.7}  & (0.4)  & \textbf{64.9}  & (1.2)  & \textbf{30.7}  & (18.5)  & \textbf{48.9}  & (6.3) \\  
%     & CS+CSAdv (Ours)        & \textbf{63.5}  & (4.7)  & \textbf{50.8}  & (6.5)  & 49.7  & (-0.6)  & 62.7  & (-1.0)  & 30.3  & (18.1)  & 48.4  & (5.8) \\ \midrule

% \multirow{5}{*}{ICNet} 
%     & CS \cite{cordts2016cityscapes}              & \textbf{61.2}  & (0.0)  & 45.4  & (0.0)  & 49.2  & (0.0)  & 64.8  & (0.0)  & 24.6  & (0.0)  & 46.0  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 38.8  & (-22.4)  & 28.3  & (-17.1)  & 33.4  & (-15.8)  & 48.0  & (-16.8)  & 16.7  & (-7.9)  & 31.6  & (-14.4) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 49.7  & (-11.5)  & 34.8  & (-10.6)  & 41.8  & (-7.4)  & 51.3  & (-13.5)  & 22.5  & (-2.1)  & 37.6  & (-8.4) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & \textbf{61.2}  & (0.0)  & 53.4  & (8.0)  & 50.3  & (1.1)  & 65.1  & (0.3)  & \textbf{38.3}  & (13.7)  & \textbf{51.8}  & (5.8) \\  
%     & CS+CSAdv (Ours)        & 59.8  & (-1.4)  & \textbf{53.4}  & (8.0)  & \textbf{50.6}  & (1.4)  & \textbf{66.1}  & (1.3)  & 35.9  & (11.3)  & 51.5  & (5.5) \\ \midrule

% \multirow{5}{*}{DDRNet} 
%     & CS \cite{cordts2016cityscapes}              & 58.4  & (0.0)  & 42.5  & (0.0)  & 48.0  & (0.0)  & 64.5  & (0.0)  & 10.6  & (0.0)  & 41.4  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 34.1  & (-24.3)  & 24.0  & (-18.5)  & 30.3  & (-17.7)  & 41.5  & (-23.0)  & 16.8  & (6.2)  & 28.2  & (-13.3) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.4  & (-10.0)  & 36.2  & (-6.3)  & 40.5  & (-7.5)  & 52.2  & (-12.3)  & 21.7  & (11.1)  & 37.7  & (-3.8) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & 59.1  & (0.7)  & 44.3  & (1.8)  & 49.0  & (1.0)  & \textbf{65.8}  & (1.3)  & \textbf{34.8}  & (24.2)  & 48.5  & (7.1) \\ 
%     & CS+CSAdv (Ours)        & \textbf{61.2}  & (2.8)  & \textbf{47.5}  & (5.0)  & \textbf{51.3}  & (3.3)  & 65.1  & (0.6)  & 34.1  & (23.5)  & \textbf{49.5}  & (8.1) \\ \midrule

% \multirow{5}{*}{CNN Average} 
%     & CS \cite{cordts2016cityscapes}              & 59.5  & (0.0)  & 44.1  & (0.0)  & 49.2  & (0.0)  & 64.3  & (0.0)  & 15.8  & (0.0)  & 43.3  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 37.6  & (-21.9)  & 26.4  & (-17.7)  & 32.5  & (-16.7)  & 45.1  & (-19.2)  & 16.2  & (0.4)  & 30.0  & (-13.3) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.5  & (-11.0)  & 35.6  & (-8.5)  & 41.3  & (-7.8)  & 51.8  & (-12.5)  & 21.4  & (5.6)  & 37.5  & (-5.8) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & 60.9  & (1.4)  & 49.0  & (4.9)  & 50.0  & (0.8)  & 65.3  & (0.9)  & 34.6  & (18.8)  & 49.7  & (6.4) \\  
%     & CS+CSAdv (Ours)        & \textbf{61.5}  & (2.0)  & \textbf{50.6}  & (6.5)  & \textbf{50.5}  & (1.4)  & 64.6  & (0.3)  & 33.4  & (17.6)  & \textbf{49.8}  & (6.5) \\ \midrule

% \multirow{5}{*}{SegFormer} 
%     & CS \cite{cordts2016cityscapes}              & 57.2  & (0.0)  & 51.2  & (0.0)  & \textbf{52.7}  & (0.0)  & 67.1  & (0.0)  & 18.5  & (0.0)  & 47.4  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 38.6  & (-18.6)  & 29.6  & (-21.6)  & 35.1  & (-17.6)  & 47.7  & (-19.4)  & 17.4  & (-1.1)  & 32.5  & (-14.9) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 46.9  & (-10.3)  & 35.6  & (-15.6)  & 42.0  & (-10.7)  & 51.0  & (-16.1)  & 22.1  & (3.6)  & 37.7  & (-9.7) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & \textbf{60.9}  & (3.7)  & \textbf{54.7}  & (3.5)  & 49.6  & (-3.1)  & \textbf{69.3}  & (2.2)  & \textbf{34.6}  & (16.1)  & \textbf{52.1}  & (4.7) \\  
%     & CS+CSAdv (Ours)        & 60.7  & (3.5)  & 53.5  & (2.3)  & 49.8  & (-2.9)  & \textbf{69.3}  & (2.2)  & 32.1  & (13.6)  & 51.2  & (3.8) \\ \midrule

% \multirow{5}{*}{Mask2Former} 
%     & CS \cite{cordts2016cityscapes}              & \textbf{67.5}  & (0.0)  & 55.4  & (0.0)  & 58.2  & (0.0)  & \textbf{73.8}  & (0.0)  & 31.4  & (0.0)  & 54.7  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 39.3  & (-28.2)  & 32.8  & (-22.6)  & 38.4  & (-19.8)  & 52.0  & (-21.8)  & 24.9  & (-6.5)  & 37.0  & (-17.7) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.4  & (-19.1)  & 39.3  & (-16.1)  & 45.1  & (-13.1)  & 53.9  & (-19.9)  & 28.3  & (-3.1)  & 41.7  & (-13.1) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & \textbf{69.8}  & (2.3)  & 61.6  & (6.2)  & \textbf{58.6}  & (0.4)  & 72.9  & (-0.9)  & 42.8  & (11.4)  & \textbf{59.0}  & (4.3) \\  
%     & CS+CSAdv (Ours)        & 68.7  & (1.2)  & \textbf{62.4}  & (7.0)  & 55.3  & (-2.9)  & 73.0  & (-0.8)  & \textbf{43.7}  & (12.3)  & 58.6  & (3.9) \\ \midrule

% \multirow{5}{*}{SETR} 
%     & CS \cite{cordts2016cityscapes}              & 60.7  & (0.0)  & 55.6  & (0.0)  & 58.3  & (0.0)  & 70.1  & (0.0)  & 38.1  & (0.0)  & 55.5  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 40.9  & (-19.8)  & 34.1  & (-21.5)  & 37.8  & (-20.5)  & 48.7  & (-21.4)  & 26.2  & (-11.9)  & 36.7  & (-18.8) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 49.1  & (-11.6)  & 40.6  & (-15.0)  & 46.2  & (-12.1)  & 52.7  & (-17.4)  & 30.5  & (-7.6)  & 42.5  & (-13.0) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & \textbf{65.5}  & (4.8)  & 61.7  & (6.1)  & 58.0  & (-0.3)  & \textbf{74.9}  & (4.8)  & \textbf{43.9}  & (5.8)  & \textbf{59.6}  & (4.1) \\  
%     & CS+CSAdv (Ours)        & 64.6  & (3.9)  & \textbf{62.2}  & (6.6)  & \textbf{59.6}  & (1.3)  & 73.9  & (3.8)  & 40.9  & (2.8)  & 59.2  & (3.6) \\ \midrule

% \multirow{5}{*}{Trans. Average} 
%     & CS \cite{cordts2016cityscapes}              & 61.8  & (0.0)  & 54.1  & (0.0)  & 56.4  & (0.0)  & 70.3  & (0.0)  & 29.3  & (0.0)  & 52.5  & (0.0) \\ \cmidrule{2-14}
%     & CSCnet \cite{loiseau2023reliability}          & 39.6  & (-22.2)  & 32.2  & (-21.9)  & 37.1  & (-19.3)  & 49.5  & (-20.9)  & 22.8  & (-6.5)  & 35.4  & (-17.1) \\  
%     & CS+CSCNet \cite{loiseau2023reliability}       & 48.1  & (-13.7)  & 38.5  & (-15.6)  & 44.4  & (-12.0)  & 52.5  & (-17.8)  & 27.0  & (-2.4)  & 40.6  & (-11.9) \\ \cmidrule{2-14}
%     & CSAdv (Ours)           & 65.4  & (3.6)  & 59.3  & (5.3)  & 55.4  & (-1.0)  & 72.4  & (2.0)  & 40.4  & (11.1)  & 56.9  & (4.3) \\  
%     & CS+CSAdv (Ours)        & \textbf{64.7}  & (2.9)  & \textbf{59.4}  & (5.3)  & \textbf{54.9}  & (-1.5)  & \textbf{72.1}  & (1.7)  & \textbf{38.9}  & (9.6)  & \textbf{56.3}  & (3.8) \\ \bottomrule

% \end{tabular}
% \end{table*}

==> tables/csadv_eval_old.tex <==
\begin{table*}
\centering
\caption{Model Performance (mIoU) with Performance Drops across Various Adverse Conditions. The table evaluates the robustness of models under different weather (rainy, foggy), seasonal (spring, autumn, snow), and lighting (sunny, night, dawn) conditions.}
\label{tab:model_performance_miou_error}
% \resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|cc|ccc|ccc|c|}
\toprule
\multirow{2}{*}{\textbf{Model Name}} & \multirow{2}{*}{\textbf{Backbone}} & \multirow{2}{*}{\textbf{Ori.}} & \multicolumn{2}{c|}{\textbf{Weathers}} & \multicolumn{3}{c|}{\textbf{Seasons}} & \multicolumn{3}{c|}{\textbf{Lightings}} & \textbf{Adverse} \\ 
& & & \textbf{Rainy} & \textbf{Foggy} & \textbf{Spring} & \textbf{Autumn} & \textbf{Snow} & \textbf{Sunny} & \textbf{Night} & \textbf{Dawn} & \textbf{Avg.} \\
\midrule
DeepLabV3+ & R-50-D8 & 80 & 58 (21) & 66 (14) & 70 (10) & 47 (33) & 22 (57) & 43 (37) & 47 (32) & 58 (22) & 51 (29) \\
ICNet & R-50-D8 & 76 & 69 (08) & 69 (07) & 71 (06) & 67 (10) & 27 (49) & 55 (22) & 61 (15) & 67 (09) & 61 (15) \\ 
DDRNet & DDRNet23 & 80 & 66 (14) & 69 (11) & 72 (08) & 55 (25) & 30 (50) & 53 (26) & 59 (21) & 65 (15) & 59 (21) \\
\cmidrule{1-12}
\multicolumn{2}{|c|}{CNN Average} & 79 & 64 (15) & 68 (11) & 71 (08) & 56 (23) & 26 (53) & 50 (29) & 56 (23) & 63 (16) & 57 (22) \\
\midrule
SegFormer & MIT-B0 & 77 & 66 (11) & 66 (11) & 69 (08) & 65 (11) & 47 (30) & 58 (19) & 63 (13) & 66 (10) & 61 (16) \\
SETR & ViT-L & 78 & 72 (06) & 71 (07) & 73 (04) & 71 (06) & 61 (16) & 62 (16) & 70 (07) & 73 (05) & 68 (10) \\ 
Mask2Former & SWIN-S & 83 & 68 (15) & 73 (10) & 75 (08) & 74 (09) & 63 (20) & 63 (20) & 69 (14) & 75 (08) & 68 (15) \\
\cmidrule{1-12}
\multicolumn{2}{|c|}{Transformer Average}& 79 & 69 (10) & 70 (09) & 72 (07) & 70 (09) & 57 (22) & 61 (18) & 67 (12) & 71 (08) & 67 (12) \\
\midrule
\multicolumn{2}{|c|}{All Average} & 79 & 66 (13) & 69 (10) & 72 (07) & 63 (16) & 42 (37) & 56 (23) & 62 (17) & 67 (12) & 62 (17) \\
\bottomrule
\end{tabular}
% }
\end{table*}

==> tables/other_datasets_eval_old.tex <==
\begin{table*}[]
\centering
\caption{Performance of CNN and Transformer-based Models Trained on Different Configurations (CS, CSAdv, and CS,CSAdv) Evaluated on Multiple Datasets. The table presents the mIoU scores for each model on each dataset and their average across all datasets.}
\label{tab:expanded-results}
% \resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
\textbf{Model Name} & \textbf{Trained On} & \textbf{bdd100k} & \textbf{dark zurich} & \textbf{night driving} & \textbf{apollo scape} & \textbf{mappilary} & \textbf{average} \\ \hline
\multirow{3}{*}{DeepLabV3+} & CS          & 37.3 & 10.3 & 20.9 & 37.3 & 38.3 & 28.8 \\  
                            & CSAdv       & 44.1 & 29.8 & 51.5 & 41.1 & 38.8 & 41.1 \\  
                            & CS,CSAdv    & 43.5 & 29.8 & 48.6 & 41.7 & 39.8 & 40.7 \\ \hline
\multirow{3}{*}{ICNet}       & CS          & 44.1 & 24.3 & 42.2 & 32.0 & 37.1 & 36.0 \\  
                            & CSAdv       & 49.2 & 37.6 & 57.0 & 36.2 & 38.8 & 43.8 \\  
                            & CS,CSAdv    & 50.4 & 36.3 & 55.0 & 35.9 & 38.7 & 43.3 \\ \hline
\multirow{3}{*}{DDRNet}      & CS          & 40.7 & 9.2  & 18.2 & 37.2 & 38.0 & 28.7 \\  
                            & CSAdv       & 46.7 & 34.3 & 52.5 & 39.6 & 38.5 & 42.3 \\  
                            & CS,CSAdv    & 46.8 & 33.5 & 52.6 & 39.6 & 39.9 & 42.5 \\ \hline
\multirow{3}{*}{SegFormer}   & CS          & 43.1 & 18.5 & 31.4 & 39.5 & 39.5 & 34.4 \\  
                            & CSAdv       & 44.6 & 32.7 & 48.1 & 37.7 & 40.4 & 40.7 \\  
                            & CS,CSAdv    & 45.0 & 31.7 & 48.6 & 38.5 & 40.3 & 40.8 \\ \hline
\multirow{3}{*}{Mask2Former} & CS          & 52.6 & 27.2 & 53.3 & 46.5 & 45.9 & 45.1 \\  
                            & CSAdv       & 54.8 & 38.0 & 61.9 & 46.4 & 46.8 & 49.6 \\  
                            & CS,CSAdv    & 55.3 & 38.5 & 65.5 & 47.2 & 46.5 & 50.6 \\ \hline
\multirow{3}{*}{SETR}        & CS          & 55.9 & 34.4 & 59.7 & 42.1 & 43.1 & 47.0 \\  
                            & CSAdv       & 56.0 & 41.6 & 61.2 & 42.0 & 44.4 & 49.0 \\  
                            & CS,CSAdv    & 55.3 & 36.8 & 60.6 & 42.0 & 44.1 & 47.7 \\ \hline
\end{tabular}
% }
\end{table*}

% \begin{table*}[]
% \centering
% \caption{Performance of CNN and Transformer-based Models Trained on Different Configurations (CS, CSAdv, and CS,CSAdv) Evaluated on BDD100K, Dark Zurich, and Night Driving Datasets. The table presents the mIoU scores for each model on each dataset and their average across all three datasets.}
% \label{tab:other-results}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|c|c|c|c|l|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{\shortstack{Model Name\\(CNN)}} & \multirow{2}{*}{Trained On} & \multicolumn{4}{c|}{Evaluation Metrics} & \multirow{2}{*}{\shortstack{Model Name\\(Transformers)}} & \multirow{2}{*}{Trained On} & \multicolumn{4}{c|}{Evaluation Metrics} \\ \cline{3-6} \cline{9-12}
%                             &                             & bdd100k & dark zurich & night driving & average &                             &                             & bdd100k & dark zurich & night driving & average \\ \hline
% \multirow{3}{*}{DeepLabV3+}  & CS                          & 37.3    & 10.3        & 20.9           & 22.8    & \multirow{3}{*}{SegFormer}  & CS                          & 43.1    & 18.5        & 31.4           & 31.0    \\ 
%                             & CSAdv                       & \textbf{44.1}    & \textbf{29.8}        & \textbf{51.5}           & \textbf{41.8}    &                             & CSAdv                       & 44.6    & \textbf{32.7}        & 48.1           & 41.8    \\ 
%                             & CS,CSAdv                    & 43.5    & 29.8        & 48.6           & 40.6    &                             & CS,CSAdv                    & \textbf{45.0}    & 31.7        & \textbf{48.6}           & \textbf{41.8}    \\ \hline
% \multirow{3}{*}{ICNet}       & CS                          & 44.1    & 24.3        & 42.2           & 36.9    & \multirow{3}{*}{Mask2Former} & CS                          & 52.6    & 27.2        & 53.3           & 44.4    \\
%                             & CSAdv                       & 49.2    & \textbf{37.6}        & \textbf{57.0}           & \textbf{47.9}    &                             & CSAdv                       & 54.8    & 38.0        & 61.9           & 51.5    \\
%                             & CS,CSAdv                    & \textbf{50.4}    & 36.3        & 55.0           & 47.2    &                             & CS,CSAdv                    & \textbf{55.3}    & \textbf{38.5}        & \textbf{65.5}           & \textbf{53.1}    \\ \hline
% \multirow{3}{*}{DDRNet}      & CS                          & 40.7    & 9.2         & 18.2           & 22.7    & \multirow{3}{*}{SETR}       & CS                          & 55.9    & 34.4        & 59.7           & 50.0    \\
%                             & CSAdv                       & 46.7    & \textbf{34.3}        & \textbf{52.5}           & \textbf{44.5}    &                             & CSAdv                       & \textbf{56.0}    & \textbf{41.6}        & \textbf{61.2}           & \textbf{52.9}    \\ 
%                             & CS,CSAdv                    & \textbf{46.8}    & 33.5        & 52.6           & 44.3    &                             & CS,CSAdv                    & 55.3    & 36.8        & 60.6           & 50.9    \\ \hline
% \end{tabular}
% }
% \end{table*}
